Does the Doer Effect Exist Beyond WEIRD Populations? Toward Analytics in Radio and Phone-Based Learning

The Doer Effect states that completing more active learning activities, like practice questions, is more strongly related to positive learning outcomes than passive learning activities, like reading, watching, or listening to course materials. Although broad, most evidence has emerged from practice with tutoring systems in Western, Industrialized, Rich, Educated, and Democratic (WEIRD) populations in North America and Europe. Does the Doer Effect generalize beyond WEIRD populations, where learners may practice in remote locales through different technologies? Through learning analytics, we provide evidence from N = 234 Ugandan students answering multiple-choice questions via phones and listening to lectures via community radio. Our findings support the hypothesis that active learning is more associated with learning outcomes than passive learning. We find this relationship is weaker for learners with higher prior educational attainment. Our findings motivate further study of the Doer Effect in diverse populations. We offer considerations for future research in designing and evaluating contextually relevant active and passive learning opportunities including leveraging familiar technology, increasing the number of practice opportunities, and aligning multiple data sources.

==> macros.tex <==

\definecolor{paleyellow}{rgb}{1, 1, 0.85}
\definecolor{lower}{rgb}{0.88235,0.7451,0.41569}
\definecolor{lower}{rgb}{0.94, 0.85, 0.6}
\definecolor{higher}{rgb}{0.5, 0.8, 0.75}
\definecolor{rowColor}{rgb}{0.937, 0.937, 0.937}
\definecolor{mauve}{rgb}{0.25,0,0.52}
\definecolor{lightpastelpurple}{rgb}{0.69, 0.61, 0.85}
\definecolor{darkolivegreen}{rgb}{0.33, 0.42, 0.18}

\newcommand{\FIXME}[1]{\textcolor{olive}{FIXME: #1}}
\newcommand{\FIXMEMLE}[1]{\textcolor{blue}{FIXME MLE: #1}}
\newcommand{\fixme}[1]{\textcolor{olive}{FIXME: #1}}

\newcommand{\subheading}[1]{\noindent\textbf{#1}}
\newcommand{\qualquote}[1]{\textit{\textcolor{mauve}{#1}}}

\newcommand{\summarytcolorbox}[1]{
\begin{tcolorbox}[colback=white, colframe=black, colbacktitle=white, coltitle=black, boxsep=0pt, top=3pt, bottom=3pt, left=6pt, right=6pt, before skip=3pt]
    \noindent #1
\end{tcolorbox}
}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}

\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}


\makeatletter
\patchcmd{\@makecaption}
  {\scshape}
  {}
  {}
  {}
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  
  
  \sbox\@tempboxa{#1. #2}%
  \ifdim \wd\@tempboxa >\hsize
    #1. #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother



